LPM effect and dielectric suppression in air showers

An analysis of the influence of the Landau-Migdal-Pomeranchuck (LPM) effect on the development of air showers initiated by astroparticles, is presented. By means of computer simulations using algorithms that emulate Migdal's theory, including also the so-called dielectric suppression, we study the behaviour of the relevant observables in the case of ultra high energy primaries. We find that the LPM effect can significantly modify the development of high energy electromagnetic showers.

==> figmacros.tex <==
\catcode`@=11
%
% Figures and tables.
%
%\def\caption{\refstepcounter\@captype \@dblarg{\@caption\@captype}}
\long\def\@caption#1[#2]#3{%
  \par
  \addcontentsline{\csname ext@#1\endcsname}{#1}%
    {\protect\numberline{\csname the#1\endcsname}{\ignorespaces #2}}%
  \begingroup
    \@parboxrestore
    \if@minipage
      \@setminipage
    \fi
    \normalsize\itshape
    \@makecaption{\bfseries\csname fnum@#1\endcsname}{\ignorespaces #3}\par
  \endgroup}
\long\def\@makecaption#1#2{%
  \vskip\abovecaptionskip
  \sbox\@tempboxa{\raggedright\parindent=0pt{\bfseries #1.} #2}%
  \ifdim \wd\@tempboxa >\hsize
    \raggedright\parindent=0pt{\bfseries #1.} #2\par
  \else
    \global \@minipagefalse
    \hb@xt@\hsize{\hfil\box\@tempboxa\hfil}%
  \fi
  \vskip\belowcaptionskip}
%
\def\rcaption{\refstepcounter\@captype \@dblarg{\@rcaption\@captype}}
\long\def\@rcaption#1[#2]#3{%
  \par
  \addcontentsline{\csname ext@#1\endcsname}{#1}%
    {\protect\numberline{\csname the#1\endcsname}{\ignorespaces #2}}%
  \begingroup
    \@parboxrestore
    \if@minipage
      \@setminipage
    \fi
    \normalsize\itshape
    \@rmakecaption{\bfseries\csname fnum@#1\endcsname}{\ignorespaces #3}\par
  \endgroup}
\long\def\@rmakecaption#1#2{%
  \vskip\abovecaptionskip
  \sbox\@tempboxa{\raggedleft\parindent=0pt{\bfseries #1.} #2}%
  \ifdim \wd\@tempboxa >\hsize
    \raggedleft\parindent=0pt{\bfseries #1.} #2\par
  \else
    \global \@minipagefalse
    \hb@xt@\hsize{\hfil\box\@tempboxa\hfil}%
  \fi
  \vskip\belowcaptionskip}
\catcode`@=12
%
% Macros for figures and tables.
%
\def\thpop{$\vphantom{|^{|^|}_{|_|}}$}
\long\def\tabcaption#1#2#3{\caption[{#2}]{\label{TAB:#1}#3}}
\long\def\figcaption#1#2#3{\caption[{#2}]{\label{FIG:#1}#3}}
\long\def\rfigcaption#1#2#3{\rcaption[{#2}]{\label{FIG:#1}#3}}
%
\long\def\lowfig#1#2#3#4#5{%
\begin{figure}#1
\begin{center}
\makebox{#3}
\end{center}
\figcaption{#2}{#4}{#5}
\end{figure}}
%
\long\def\latfig#1#2#3#4#5{%
\begin{figure}#1
\begin{flushright}
\makebox{\makebox{#3}\kern 1em
\parbox[b]{0.3\textwidth}{\figcaption{#2}{#4}{\strut #5\strut}}}
\end{flushright}
\end{figure}}
%
\long\def\rlatfig#1#2#3#4#5{%
\begin{figure}#1
\begin{flushleft}
\makebox{\parbox[b]{0.3\textwidth}%
{\rfigcaption{#2}{#4}{\strut #5\strut}\kern 1em}\makebox{#3}}
\end{flushleft}
\end{figure}}
%
\long\def\lowtable#1#2#3#4#5{%
\begin{table}#1
\begin{center}
\makebox{#3}
\end{center}
\tabcaption{#2}{#4}{#5}
\end{table}}
%
\long\def\lattable#1#2#3#4#5{%
\begin{table}#1
\begin{flushright}
\makebox{\makebox{#3}\kern 1em
\parbox[b]{0.3\textwidth}{\tabcaption{#2}{#4}{\strut #5\strut}}}
\end{flushright}
\end{table}}
%
% And some related parameters...
%
\setcounter{topnumber}{1}
\renewcommand{\topfraction}{0.8}
\setcounter{bottomnumber}{1}
\renewcommand{\bottomfraction}{0.8}
\setcounter{totalnumber}{20}
\renewcommand{\floatpagefraction}{0.0}

